Exploring Concept Depth: How Large Language Models Acquire Knowledge and Concept at Different Layers?

Large language models (LLMs) have shown remarkable performances across a wide range of tasks. However, the mechanisms by which these models encode tasks of varying complexities remain poorly understood. In this paper, we explore the hypothesis that LLMs process concepts of varying complexities in different layers, introducing the idea of "Concept Depth" to suggest that more complex concepts are typically acquired in deeper layers. Specifically, we categorize concepts based on their level of abstraction, defining them in the order of increasing complexity within factual, emotional, and inferential tasks. We conduct extensive probing experiments using layer-wise representations across various LLM families (Gemma, LLaMA, Qwen) on various datasets spanning the three domains of tasks. Our findings reveal that models could efficiently conduct probing for simpler tasks in shallow layers, and more complex tasks typically necessitate deeper layers for accurate understanding. Additionally, we examine how external factors, such as adding noise to the input and quantizing the model weights, might affect layer-wise representations. Our findings suggest that these factors can impede the development of a conceptual understanding of LLMs until deeper layers are explored. We hope that our proposed concept and experimental insights will enhance the understanding of the mechanisms underlying LLMs. Our codes are available at https://github.com/Luckfort/CD.

==> body/6discussion.tex <==
\section{Discussion}

Probing technology can potentially revolutionize various aspects of inference in large language models. One exciting application involves using probes to determine the layer at which a concept is learned within a neural network in an LLM. This information can then be leveraged to perform targeted model pruning, specifically removing the layers that follow the identified layer. These probes act as detectors, identifying the layers where specific concepts or features are learned. This knowledge allows us to identify the critical layers that contribute significantly to the model's final predictions. Once the layer responsible for learning a particular concept is identified, targeted model pruning can be applied. Pruning involves removing unnecessary or less influential layers from the network while preserving its overall performance. By cutting off the layers that follow the identified important layer, we eliminate computation costs and reduce the model's complexity, resulting in faster inference times. 

==> table/table.tex <==
\begin{table}
        \caption{The datasets in each task.}
	\centering
	\begin{tabular}{|c|c|c|c|}
		\hline
		\multirow{I} & II & III & IV \\
		\cline{2-4}
		~ & 2 & 3 & 4 \\ \cline{2-4}
            ~ & 2 & 3 & 4 \\
		\hline
	\end{tabular}
\end{table}
